Affine deformations of a three-holed sphere

Associated to every complete affine 3-manifold M with nonsolvable fundamental group is a noncompact hyperbolic surface S. We classify such complete affine structures when Sigma is homeomorphic to a three-holed sphere. In particular, for every such complete hyperbolic surface Sigma, the deformation space identifies with two opposite octants in R^3. Furthermore every M admits a fundamental polyhedron bounded by crooked planes. Therefore M is homeomorphic to an open solid handlebody of genus two. As an explicit application of this theory, we construct proper affine deformations of an arithmetic Fuchsian group inside Sp(4,Z).

==> Makefile <==
# makefile for affineths
# last modified 052508 in Kortrijk

MASTERFILE 	= affineths.tex
MAKEFILE	= Makefile
OTHERTEXT	= affineths.toc affineths.aux affineths.log affineths.dvi
DVIFILE		= affineths.dvi
PDFFILE		= affineths.pdf
PICTUREFILES	= OSspace.pstex   SEspace.pstex   hexagon.pstex    hexagonII.pstex   threelines.pstex \
		  OSspace.pstex_t SEspace.pstex_t hexagon.pstex_t  hexagonII.pstex_t threelines.pstex_t \
		  idealpattern1.pstex idealpattern1.pstex_t  idealpattern2.pstex idealpattern2.pstex_t 
SOURCE 	= $(MASTERFILE) $(OTHERSOURCEFILE) $(PICTUREFILES)
EVERYTHING 	= $(SOURCE) $(PDFFILE) $(MAKEFILE)

affineths:	$(SOURCE)
	latex $(MASTERFILE)
	latex $(MASTERFILE)
	latex $(MASTERFILE)
	dvipdf $(DVIFILE)
dvi:	$(SOURCE)
	latex $(SOURCE)

# preview on the screen
view:	$(PDFFILE)
	open $(PDFFILE)

# remove auxiliary files, including .dvi
clean:	$(OTHERTEXT)
	rm $(OTHERTEXT)

# create archive file, useful for emailing and backup
tar:	
	tar cvzf ../CharetteDrummG.tar.gz ../src 
# creates compressed tar files with all source files
# including Makefile, .tex source and all graphics
# and the pdf

# unpack archive file
untar:	
	tar xvf CharetteDrummG.tar.gz
# to untar: tar xvf CharetteDrummG.tar.gz
# creates directory named "src" with all files
# view .pdf with "make view" from this directory

# I don't know if we need anything else after this
#
# backup on MathNet
umd:	$(SOURCE)
	scp $(SOURCE) noether.math.umd.edu:CharetteDrummG/src

# convert .dvi file to .pdf
pdf:	$(DVIFILE) 
	dvipdf $(DVIFILE)

MISCPICTUREFILES = 
FIGURES 	 =




